Optimal Indexes for Sparse Bit Vectors

We consider the problem of supporting Rank() and Select() operations on a bit vector of length m with n 1 bits. The problem is considered in the succinct index model, where the bit vector is stored in "read-only" memory and an additional data structure, called the index, is created during pre-processing to help answer the above queries. We give asymptotically optimal density-sensitive trade-offs, involving both m and n, that relate the size of the index to the number of accesses to the bit vector (and processing time) needed to answer the above queries. The results are particularly interesting for the case where n = o(m).

==> abstract.tex <==
We consider the problem of supporting $\Rank{}$ and $\Select{}$ operations on
a bit vector of length $m$ with $n$ 1 bits.  The problem is considered in 
the \emph{succinct index} model, 
where the bit vector is stored in ``read-only'' memory and an additional data structure,
called the \emph{index} is created during pre-processing to help answer the above queries.
We give asymptotically optimal density-sensitive trade-offs, involving both $m$ and $n$,
that relate the size of the index to the number of accesses to the bit vector 
(and processing time) needed to answer the above queries. The results are particularly interesting
for the case where $n = o(m)$.



==> conclusions.tex <==
\section{Conclusions}

We have provided matching density-sensitive 
upper and lower bounds on the redundancy required for
\Rank{} and \Select{} operations on sparse bit vectors in the {succinct index} model.
These results improve signficantly on known results 
for the case where $n = o(m)$.  Although our results depend on both $m$ and $n$, we
do not take into account any regularities in the distribution of 1s in the bit vector; 
an interesting direction of research would be to find appropriate measures of the
regularities of 1s in the bit vector that could lead to further reductions in the
index size.

